Multimodal Interaction with Multiple Co-located Drones in Search and Rescue Missions

We present a multimodal interaction framework suitable for a human rescuer that operates in proximity with a set of co-located drones during search missions. This work is framed in the context of the SHERPA project whose goal is to develop a mixed ground and aerial robotic platform to support search and rescue activities in a real-world alpine scenario. Differently from typical human-drone interaction settings, here the operator is not fully dedicated to the drones, but involved in search and rescue tasks, hence only able to provide sparse, incomplete, although high-value, instructions to the robots. This operative scenario requires a human-interaction framework that supports multimodal communication along with an effective and natural mixed-initiative interaction between the human and the robots. In this work, we illustrate the domain and the proposed multimodal interaction framework discussing the system at work in a simulated case study.

==> section/case-studies.tex <==
% Descrition of real and simulated case studies

\subsection{Experimental Set-up}
The operator is equipped with headset (speech), Xsens MVN biomech suite (gestures) and a tablet to communicate with the drones.

\subsection{Simulated Environment}
Two Drones (Asctec Pelican) simulated in the Unity 3D game engine. 


\subsection{Lab Environment}
Lab. Environment: three CrazyFly quadcopters tracked by an optitrack motion capture system.

==> section/mixed-multimodal.tex <==
The human operator should interact with the robots in a simple and intuitive manner, focusing the cognitive effort on relevant and critical activities (e.g. visual inspection, precise maneuvering, etc.) while relying on the robotic autonomous system for routinized operations and behaviors.  Therefore, the robotic architecture should support different control modes form the autonomous one to direct teleoperation passing through the \textit{mixed-Initiative} mode, where the user can execute some operations while relying on the autonomous control system for the remaining ones.

\subsection{Multimodal Mixed-Initiative Interaction Architecture}

We designed a modular architecture suitable for supervising and orchestrating the activities of both groups of robots and single robots. The operator should be capable of interacting with the system using different modalities (joypad, gestures, speech, tablet, etc.) at different levels of abstraction
(task, activity, path, trajectory, motion, etc.). These continuous human interventions are to be suitably and reactively interpreted and integrated in the robotics control loops providing a natural and intuitive interaction.  The architecture of our HRI system is illustrated in Figure \ref{fig:completearch}, in the following we illustrate each component.
\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.45]{./Figure/arch_sup_3_NEW.png}
		\par
		\caption[Complete Architecture]{The overall HRI architecture}
		\label{fig:completearch}
	\end{center}
\end{figure} 

%The integration of different modalities permits a natural, flexible, and robust communication between the human and the system.
The multimodal interaction block allows the human operator to interact with the drones through speech, gestures, tablet interfaces interpreting the underlying intention. For instance, while the voice commands concern movement, selection, and exploration commands, gesture-based communication can be used to specify navigational commands with deictic communication (e.g. {\em go-there}) during a proximity interaction with the co-located drones. Notice that commands can be given at different levels of abstraction, from task assignments  to direct teleoperation (see Table \ref{tab:voice_gesture_command}). 
As for teleoperation, gestures can be used also as joypad-like control commands to manually guide the robots or to adjust the execution of specific tasks. For instance, the operator may want to modify the robots orientation or elevation, without changing the robot task. Beyond line-of-sight control, feedback from the drones can be provided via a tablet interface and headphones.

The sketchy and abstract inputs of the human are further interpreted by the mixed-initiative module (MI) that interacts with the single robot supervisor (SRS)  and multirobot supervisors (MRS) mediating between the human and the robotic initiative. For instance, commands can be provided to both single or multirobots, and sketchy instructions are to be completed and instantiated by the robots supervisory systems. In our framework, both the MRS and the SRS are endowed with a BDI executive engine \cite{Ingrand92} and a task/path/motion planners to support mixed-initiative control and sliding autonomy. Indeed, following a mixed-initiative planning approach \cite{Finzi05} the human interventions are integrated into continuous planning and execution processes that reconfigure the robotic activities according to the human intentions and the operative state. 
%A detailed description of this system is beyond the scope of this
%paper that focuses on multimodal interaction aspects. 
   
\begin{table}[h]
	\caption{Voice and Gesture commands}
		\begin{center}
		\begin{tabular}{|c|c|}			
			\hline
			%---Title---%
			\textbf{Command} 		&  \textbf{Source} \\
			\hline
			%---Commands---%
			\textit{Take-Off} 		& Voice\\			
			\hline	
			\textit{Continue} 		& Voice\\			
			\hline	
			\textit{Land} 			&  Voice\\			
			\hline	
			\textit{Rotate \$o'clock}   &  Voice \\
			\hline	
			\textit{Selection \$Drone-Id}   &  Voice  \\
			\hline	
			\textit{Distance size}   &  Voice \\
			\hline	
			\textit{Faster}   &  Voice and Gesture \\
			\hline	
			\textit{Slower}   &  Voice and Gesture \\
			\hline			
			\textit{Rotate Clockwise} &  Gesture\\
			\hline	
			\textit{Rotate Anti-clockwise} &  Gesture\\
			\hline					
			\textit{Brake} 			& Voice and Gesture\\			
			\hline	
			\textit{Go \$Direction}  &  Voice and Gesture\\
			\hline	
			\textit{Search Expanding}   &  Voice and Gesture \\
			\hline	
			\textit{Search Parallel Track}   &  Voice and Gesture \\
			\hline	
			\textit{Search Creeping Line}   &  Voice and Gesture \\
			\hline
			\textit{Direction Pointing}   &  Voice and Gesture \\
			\hline									
		\end{tabular}
		\label{tab:voice_gesture_command}
		\end{center}
\end{table}

%Different modalities can be simultaneously used even if they export the same information. This redundancy can be useful to help the system in the fusion phase and to avoid errors in input signals.
%
%

\subsection{Multimodal Interaction}
%In multimodal interaction framework, data coming from the different channels have to be integrated to produce a single interpretation for a t	ask, command, or query. 
We refer to a multimodal interaction framework that exploits a late fusion approach \cite{iros2013} where single modalities are separately classified and then combined (see Figure \ref{fig:multimodal}).
\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.4]{./Figure/IROS2015_fusion.png}
		\par
		\caption[Multimodal Architecture]{Multimodal Interaction System}
		\label{fig:multimodal}
	\end{center}
\end{figure} 

In this work, we mainly focus on commands suitable for interacting with a set of drones, co-located with the human operator, during navigation and search tasks. 
%In particular, we focus on speech and gestures. The operator can communicate with the drones using only vocal high-level commands, e.g. ”all hawks take off”, or only gestures (e.g. gestures for $stop$ and $search$), or by combining voice and gestures. In this modality voice, can be used to specify a high level commands, while gestures can add information or vice-versa. For example, if the operator wants to move the robot towards a desired location, he can use a gesture the select the command while using the voice to specify the distance to travel. In the same way, high level commands generated by the voice can be modified by gestures.
%Note also that, in the challenging domain we are concerned with, the multimodal interaction provide redundancy that should improve the robustness of the overall communication between the operator and the drones. 
In particular, we are concerned with speech- and gestures-based communication with the drones suitable for the following purposes:
\begin{itemize}
\item
{\em Selection:} in order to select single or groups of robots involved in the action, both speech (e.g. ”all hawks take off”, ”red hawks land”) and gestures (e.g. ”you go down”) can be used in combination. Specific names (”red hawk”, ”blue hawk”, etc.) can identify drones, while deictic gestures (pointing) can be used to select not only drones, but also targets (e.g. ”you go there”).
%A unique identifier (voice) or a deictic  command (gesture) can be used for this purpose. 
%In this case, a composition of voice and gesture is necessary.
%\item
%{\em Atomic action:} a set of commands are used for atomic actions such as {\em Take-off} or {\em Land}.
\item
{\em Motion:} a set of commands are used for navigation (see Table \ref{tab:voice_gesture_command}) %, namely, {\em take-off}, {\em land}, {\em go-there},
%{\em go-ahead}, {\em go-backward}, {\em go-up}, {\em go-down}, {\em go-left}, {\em go-right},  {\em rotate}. 
Motion directives can be coupled with voice directives. In particular, a rotation command can be associated with the final orientation of the drone, while in the movement commands the operator can specify the exact distance to be covered. When these values are not explicitly provided, default ones are assumed.
\item
{\em Search:} a set of commands are used to select the search pattern used to scan an area with a helicopter search \cite{NATO-88}, i.e. search-expanding, search-parallel-track and search-creeping-line (see Figure \ref{fig:search_patterns}). 
\item 
{\em Switch:} meta level commands allow the operator to change the interaction mode and metaphor, e.g. from command-based to joypad-like interactive control.
%These search strategies are inspired by the one proposed by ... 
%(definire in che situazione si usa un search pattern in accordo con il manuale di S\&R ? ).
\end{itemize}

\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.06]{./Figure/Searching_patterns.png}
		\par
		\caption[searching_patterns]{Parallel Track (Left), Expanding (Center) and Creeping Line (Right) search patterns}
		\label{fig:search_patterns}
	\end{center}
\end{figure} 

In Table \ref{tab:voice_gesture_command}, we propose a set of commands which can be flexibly combined and invoked during multimodal interaction with speech and gestures. As for speech recognition, we rely on Julius\cite{julius01}, a two-pass large vocabulary continuous speech recognition (LVCSR) engine. 
In the following, we provide details about the adopted methods for speech, gesture recognition, and late fusion. 
%[Aggiungere qualche info su julius??]
%Moreover, different metaphors of interaction can be deployed while interacting with the drones. 

%Prima: voce e gesti di alto livello e basso livello e composizione di essi
\paragraph*{Speech recognition} we rely on Julius\cite{julius01}, a two-pass large vocabulary continuous speech recognition (LVCSR) engine. 
A simple grammar has been defined to parse simple commands of the users. A N-best list of possible interpretations is continuously provided in
output.   

\paragraph*{Gestures recognition}
%%Descrizione myo talmich
Our gesture recognition system exploits the {\em Thalmic Myo Armbend}. This device allow us to detect and distinguish several poses of the hand (see Figure \ref{fig:myo_poses}) from the electrical activity of the muscles of the arm where the band is weared. In addition, 
the band is endowed with a 9 $DOF$ IMU that permits motion capture. Therefore, both hand poses and movements
can be detected and used for the robot control. 
In our framework, the position of the hand can be used to enable/disable control modalities ({\em switch} commands), while
the movements of the hand are to be interpreted as gestures.
\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.35]{./Figure/myo_poses.png}
		\par
		\caption[myo poses]{Different poses of the hand recognized by Thalmic Myo Armbend}
		\label{fig:myo_poses}
	\end{center}
\end{figure} 
%introduzione gesture recognition con Myo
%measures the accelerations and by electrical activity of the muscles captured by Myo Armband devices. 
%We exploit these two data channels to classify two kind of gestures. 
As far as the hand poses are concerned, we directly rely on the built-in {\em Myo Armband} classifiers. Instead, we exploit a device independent classification method for the arm movements. Specifically, our approach is inspired by  \cite{kratz2010}, which has the advantage that only simple geometric methods are necessary to classify. Moreover, since in our scenario we assume the presence of a trained operator (the busy genius), a user-dependent gesture recognition method is satisfactory, and in this case, the proposed method requires only few samples for training. On the other hand, the main problem of this approach is that it does not support continuous recognition: for each gesture the classifiers needs the start and and the end.  
%and could give better result for in the case of a non-general application. %da migliori risultati a chi ha registrato il data set rispetto gli standard approcci probabilistici
We address this problem exploiting the hand pose detected by the {\em Myo Armband} classifiers, i.e. we assume that the trajectory of a gesture is tracked
and classified when the hand is closed. 
%I each gestures performed with the closed hand can be interpreted by the classifiers. 
%filtraggio segnale ingresso
Once the gesture trajectories are delimited, the gesture classification process works as follows. Initially, two transformations are deployed to filter the acceleration signal generated by the device. The first one rotates the acceleration data from world frame to sensor frame to make the gesture independent from the position of the arm of the user. The second one is used to remove noise from the acceleration sample set deleting all the acceleration $\vec a_i$ for wich $| \vec a_i - \vec a_{i-1} | < \epsilon $. 
%Riconoscimento del gesto
In the second place, the input signal is resampled into a fixed number of points describing the gesture trajectory. This process allows us to compare the input gesture with respect to the input gestures in the dataset according to an euclidean distance which is used to produce a $N$-best list of the best matches with a unique gestures. 
%Aggiungere second recognition phase
This simple recognition process is further improved by a secondary evaluation process which takes into account the orientation of a gesture. More specifically, when the differences between the last $2$-best values is below a suitable threshold, the gestures are ranked again by improving the values of the gestures whose average orientation is closer to the average orientation of the performed gesture (???). %PS non mettiamo l'orientamento come grado di liberta perche non è detto che fornisca esattamente una buona classificazione e appesentirebbe inutilmente il riconoscitore
%sliding windows 
In addition, in order to reduce the delay of the classification, different instances of the recognizer run in parallel checking for the best matching within a sliding window that crop the initial samples of the input gesture (e.g. Figure  \ref{fig:sliding_window_gr} illustrates $3$ instances running).
%evaluation

As for the dataset, we defined $14$ different types of gestures for both  navigation commands and search strategy requests. We evaluated the gesture recognizer by performing $30$ trial of all gestures (randomly to avoid the learning effect). In Table \ref{tab:gesture_classification_res} we report \textit{Precision}, \textit{Recall} and \textit{Accuracy} for all gestures of the training set. The training set of the evaluation system is obtained from $10$ examples of the same gesture (one for each trained operator).

\begin{figure}[h]
	\begin{center}
		\includegraphics[scale=0.18]{./Figure/gr_window.png}
		\par
		\caption[Sliding Windows GR]{Gesture matching at different time (start, middle, end) of the sliding window. Dashed and solid curves represents the recognized and executed gesture respectively.}
		\label{fig:sliding_window_gr}
	\end{center}
\end{figure} 


%%--- Risultati classificatore gesti con solo "Precision, recall, accurcy"
\begin{table}[h]
	\caption{Gesture classification results}
		\begin{center}
		\begin{tabular}{|c||c||c|c||}
			\hline
			%---Title---%
			\textbf{Gesture} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy}\\
			\hline
			%---Datas---%
			\textit{Brake} & 93.3\% & 96.5\% & 94.9\% \\
			\hline			
			\textit{Go Ahead} & 96.6\% & 90.6\% & 93.4\% \\
			\hline
			\textit{Go Backward} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Down} & 100\% & 88.3\% & 93.5\% \\
			\hline
			\textit{Go Left} & 73.3\% & 100\% & 86.2\% \\
			\hline
			\textit{Go Right} & 96.6\% & 85.3\% & 90.4\% \\
			\hline
			\textit{Go Up} & 100\% & 96.7\% & 98.3\% \\
			\hline
			\textit{Rotate Anti-Clockwise} & 100\% & 96.7\% & 98.3\% \\
			\hline
			\textit{Rotate Clockwise} & 83.3\% & 100\% & 91.38\% \\
			\hline
			\textit{Search Creeping Line} & 80\% & 82.7\% & 82.4\% \\
			\hline
			\textit{Search Expanding} & 96.6\% & 85.3\% & 90.4\% \\
			\hline
			\textit{Search Parallel Track} & 96.6\% & 90.6\% & 93.4\% \\
			\hline
			\textit{Faster} & 96.6\% & 82.9\% & 88.9\% \\
			\hline
			\textit{Slower} & 66.6\% & 90.9\% & 79.9\% \\
			\hline
			\hline
			\textit{Average} & 91.4\% & 91.9 \% & 91.7 \% \\
			\hline
		\end{tabular}
		\label{tab:gesture_classification_res}
	\end{center}
\end{table}
%---
%-----Risultati classificatore con le percentuali di TP FP TN e FN
%\begin{table}[h]
%	\caption{Gesture classification results}
%		%\begin{center}
%		\begin{tabular}{|c||c||c||c||c||c||c|c|}
%			\hline
%			%---Title---%
%			\textit{Gesture} & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{Precision} & \textit{Recall} & \textit{Accuracy}\\
%			\hline
%			%---Datas---%
%			Brake & 93.3333\% & 6.66667\% & 92.619\% & 3.33333\% & 93.3333\% & 96.5517\% & 94.8967\% \\
%			\hline
%			Faster & 96.6667\% & 3.33333\% & 91.4286\% & 20\% & 96.6667\% & 82.8571\% & 88.964\% \\
%			\hline
%			Go Ahead & 96.6667\% & 3.33333\% & 92.1429\% & 10\% & 96.6667\% & 90.625\% & 93.404\% \\
%			\hline
%			Go Backward & 100\% & 0\% & 92.8571\% & 0\% & 100\% & 100\% & 100\% \\
%			\hline
%			Go Down & 100\% & 0\% & 91.9048\% & 13.3333\% & 100\% & 88.2353\% & 93.5035\% \\
%			\hline
%			Go Left & 73.3333\% & 26.6667\% & 92.8571\% & 0\% & 73.3333\% & 100\% & 86.1728\% \\
%			\hline
%			Go Right & 96.6667\% & 3.33333\% & 91.6667\% & 16.6667\% & 96.6667\% & 85.2941\% & 90.4\% \\
%			\hline
%			Go Up & 100\% & 0\% & 92.619\% & 3.33333\% & 100\% & 96.7742\% & 98.2989\% \\
%			\hline
%			Rotate Anti-Clockwise & 100\% & 0\% & 92.619\% & 3.33333\% & 100\% & 96.7742\% & 98.2989\%  \\
%			\hline
%			Rotate Clockwise & 83.3333\% & 16.6667\% & 92.8571\% & 0\% & 83.3333\% & 100\% & 91.358\% \\
%			\hline
%			Search Creeping Line & 80\% & 20\% & 91.6667\% & 16.6667\% & 80\% & 82.7586\% & 82.4\% \\
%			\hline
%			Search Expanding & 96.6667\% & 3.33333\% & 91.6667\% & 16.6667\% & 96.6667\% & 85.2941\% & 90.4\% \\
%			\hline
%			Search Parallel Track & 96.6667\% & 3.33333\% & 92.1429\% & 10\% & 96.6667\% & 90.625\% & 93.404\% \\
%			\hline
%			Slower & 66.6667\% & 33.3333\% & 92.381\% & 6.66667\% & 66.6667\% & 90.9091\% & 79.9043\% \\
%			\hline
%
%		\end{tabular}
%		\label{tab:gesture_classification_res}
%	%\end{center}
%\end{table}


%%--- Risultati classificatore gesti con solo "Precision, recall, accurcy"
\begin{table}[h]
	\caption{Multimodal results}
		\begin{center}
		\begin{tabular}{|c||c||c|c||}
			\hline
			%---Title---%
			\textbf{Gesture} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy}\\
			\hline
			%---Datas---%
			\textit{Brake} & 80\% & 100\% & 88.8\% \\
			\hline
			\textit{Faster} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Ahead} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Backward} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Down} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Left} & 80\% & 100\% & 88.8\% \\
			\hline
			\textit{Go Right} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Go Up} & 100\% & 83.3\% & 89.85\% \\
			\hline
			\textit{Rotate Anti-Clockwise} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Rotate Clockwise} & 97.3\% & 83.3\% & 91.38\% \\
			\hline
			\textit{Search Creeping Line} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Search Expanding} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Search Parallel Track} & 100\% & 100\% & 100\% \\
			\hline
			\textit{Slower} & 100\% & 83.3\% & 89.8\% \\
			\hline
			\hline
			\textit{Average}:  & 96.95\% & 96.4\% & 96.3\%\\
			\hline

		\end{tabular}
		\label{tab:gesture_classification_res}
	\end{center}
\end{table}

\paragraph*{Late Fusion}
The aim of the {\em fusion module} is to combine the results of vocal and/or gesture recognition into a uniform interpretation using. We deploy a late fusion approach that exploits the confidence values associated with the single modalities. In this direction, contextual rules are used to \textit{disambiguate} the conflicting commands or to \textit{combine} vocal and gesture input using the information contained in both the channels.  In the first case, or when an explicit rule is not available, the $N$-best values provided by the voice and gesture recognizers are compared and the interpretation with the maximum value is selected. %For example if both voice and gesture provide as best result a High Level command (i.e \textit{Go Ahead} and \textit{Go Left} ), the final command is generated searching an unique element contained in both lists that maximize the recognition confidence. 
In the second case, if the classification results are compatible, these are combined according to simple rules (e.g. navigation gesture towards a certain direction combined with a vocal indication of a distance is interpreted as \textit{Go to \$distance}). Table \ref{tab:gesture_classification_res} illustrates the improved classification results due to the fusion engine.

%is illustrated in Figure \ref{fig:multimodal}. 
%rifare grafico figura... aggiungere qualcosa?

\subsection{Mixed-Initiative Interaction}
The operator is always allowed to interact with the drones at different levels of abstraction, while using different interaction metaphors \cite{PfeilKL13}.  
The task-level mixed-initiative interaction is illustrated in \cite{icaps-15}, in this work we are mainly concerned with path/trajectory level interaction.  
In particular, we distinguish between {\em command-based} and {\em joypad-based} interaction. In the latter modality, the operator hand can be used as
a virtual joystick to teleoperate the selected drones or to adjust the planned trajectories. In order to switch to this interaction metaphor, we use 
the hand position: when the hand is closed ({\em hand-closed} mode), also already explained, the arm movement is interpreted as a gesture-based command, 
otherwise, when the hand is open  ({\em hand-open} mode), it is interpreted as a joypad-based command for the selected drone. For instance, the human may ask a drone the execution of a task (e.g. ``blue hawks go there''), and once the execution starts use the {\em hand-open} mode to correct the trajectory. A full {hand-open} teleoperation can be reached once the current command execution has been stopped with a  {\em brake}.   
%switch the drone operations to an autonomous, mixed-initiative, or teleoperated mode. Moreover, the human is allowed to select one of the drones or all them and assign or modify a task, modify a path or a trajectory, or directly teleoperate the selected drone/drones.  

%At lower level of abstraction the operator can controls drones in mixed-initiative paradigm as described in \cite{iros14}. 
%When the mixed-initiative control modality is active, the human operator can operate some interventions while the drones execute a task. 

% {\em Multimodal navigation control.} 
 
% {\em Path/trajectory deviation.} 
  %path/trajectory level, the human can deviate from 

%At the lower level, as described in \cite{iros14}, the human form the planned trajectory is possible 	$a_C(t)$ as the position commanded at time $t$ byautonomous system and $h_C(t)$ the relative position command  at time $t$, generated by the human operator the final control input sent to there robot is
%\begin{center}
%			$h_C$(t) = $\begin{cases}
%			h_C(t-1)+human(t) $ if $ mixed=ON\\
%			h_C(t-1)+\Lambda(t) $  $ otherwise
%		\end{cases}$
%\end{center}
%where $teleoperation(t)$ represents the data generated by the human operator through the remote device at time $t$ and $\Lambda(t)$ is a linear function that increases or decreases the value of $h_C(t)$ to drive the $h_C(t)$ towards the position generated by the autonomous control. 

%\paragraph*{Command-based interaction} 
%In fact the operator can use both voice and gesture to specify the same command...
%Mixed initiative
%The multimodal interaction permits even the control of the robots via the Mixed-initiative paradigms, in which the autonomous system of the robot and the human operator collaborates for the accomplishment of the mission.
%Pure teleoperation
%In the end at lower level of abstraction, the user operator can control a drone in purely teleoperation, sending input control to the robot using the Armband device.
%\\
%\textbf{...Discussione su switching di modalità operative? Per come è l'architettura basta modificare la posa della mano per modificare la modalità operativa...}

%---Gestures recignition

%

\paragraph*{Path and Trajectory level interaction.}
The navigation commands introduced so far are associated with drone movements to be suitably planned and executed.
We deploy an $RRT^*$ algorithm \cite{Karaman.Frazzoli:RSS10} for path planning, while trajectory planning is based on a 4$-th$ order spline concatenation preserving continuous acceleration. Following the approach in \cite{iros14}, the human is allow to on-line adjust the robot planned trajectory without replanning. More specifically, the operator can generate a relative position command $h_C(t)$ $=$ ($x_{m_t}, y_{m_t}, z_{m_t}$) that is added to $a_C$ $=$ ($x_t, y_t, z_t$) generated by the trajectory planner.  The $h_C$ function is calculated as follows:
\begin{center}
			$h_C$(t) = $\begin{cases}
			h_C(t-1)+human(t) $ if $ mixed=ON\\
			h_C(t-1)+\Lambda(t) $  $ otherwise
		\end{cases}$
\end{center}
where $human(t)$ represents the control reference generated by the human operator (via gestures or voice) at time $t$. 
while $\Lambda(t)$ is a linear function that increases or decreases the value of $h_C(t)$. It is used to drive the $h_C(t)$ towards the one provided by the autonomous control when the human intervention is released (see \cite{iros14} for an analogous approach). 
%
%
Moreover, as in \cite{iros14}, we assume that the human operator can move the robot within a spherical region, representing a workspace, centered in the current planned position. A replanning process (analogous to the one used for obstacle avoidance) is started when the human operator moves the robot out of this sphere. In this case, the autonomous system generates another path and trajectory to reach the next waypoint. Differently from \cite{iros14}, instead of force-feedback, a vibration-based feedback is provided to signal to the user when a replanning process is going to be invoked. 
